Two-particle correlations in azimuthal angle and pseudorapidity in central $^7$Be+$^9$Be collisions at the CERN Super Proton Synchrotron

A measurement of charged hadron pair correlations in two-dimensional $\Delta\eta\Delta\phi$ space is presented. The analysis is based on total 30 million central Be+Be collisions observed in the NA61/SHINE detector at the CERN SPS for incident beam momenta of 19$A$, 30$A$, 40$A$, 75$A$, and 150$A$ GeV/$c$. Measurements were carried out for unlike-sign and like-sign charge hadron pairs independently. The $C(\Delta\eta,\Delta\phi)$ correlation functions were compared with results from a similar analysis on p+p interactions at similar beam momenta per nucleon. General trends of the back-to-back correlations are similar in central Be+Be collisions and p+p interactions, but are suppressed in magnitude due to the increased combinatorial background. Predictions from the EPOS and UrQMD models are compared to the measurements. Evolution of an enhancement around $(\Delta\eta,\Delta\phi) = (0,0)$ with incident energy is observed in central Be+Be collisions. It is not predicted by both models and almost non-existing in proton-proton collisions at the same momentum per nucleon.

==> tables/cuttable_events_short.tex <==
\begin{tabular}{|l|c|c|}
\hline
	 & Interactions & Selected events \\
\hline
19 GeV/c & 565136 & 29531 (5.2\%)\\
30 GeV/c & 647662 & 38550 (6\%)\\
40 GeV/c & 1833013 & 109512 (6\%)\\
75 GeV/c & 2030413 & 92741 (4.6\%)\\
150 GeV/c & 1644127 & 81525 (5\%)\\
\hline
\end{tabular}

